Constrained Power Reference Control for Wind Turbines

The cost of wind energy can be reduced by controlling the power reference of a turbine to increase energy capture, while maintaining load and generator speed constraints. We apply standard torque and pitch controllers to the direct inputs of the turbine and use their set points to change the power output and reduce generator speed and blade load transients. A power reference controller increases the power output when conditions are safe and decreases it when problematic transient events are expected. Transient generator speeds and blade loads are estimated using a gust measure derived from a wind speed estimate. A hybrid controller decreases the power rating from a maximum allowable power. Compared to a baseline controller, with a constant power reference, the proposed controller results in generator speeds and blade loads that do not exceed the original limits, increases tower fore-aft damage equivalent loads by 1%, and increases the annual energy production by 5%.

==> Constrained Power Reference Control for Wind Turbines/Lato-fonts/Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree


==> Lato-fonts/Makefile <==
## Makefile
## Copyright 2011 Mohamed El Morabity
#
# This work may be distributed and/or modified under the conditions of the LaTeX
# Project Public License, either version 1.3 of this license or (at your option)
# any later version. The latest version of this license is in
# http://www.latex-project.org/lppl.txt and version 1.3 or later is part of all
# distributions of LaTeX version 2005/12/01 or later.
#
# This work has the LPPL maintenance status `maintained'.
#
# The Current Maintainer of this work is Mohamed El Morabity
#
# This work consists of all files listed in manifest.txt.

######################
# Fonts informations #
######################

FONT_NAME = lato
FOUNDRY = public
FONT_CODES = fla

# Supported LaTeX encodings
SUPPORTED_ENCODINGS = ot1 t1 ts1
# Supported LaTeX encodings containing small caps
SUPPORTED_SC_ENCODINGS = $(filter-out ts1,$(SUPPORTED_ENCODINGS))
# Custom encodings provided
INPUT_ENCODINGS = $(INPUT_ETX_FILES:$(FONT_NAME)-%.etx=%)


#####################
# Installation root #
#####################

TEXMFHOME = $(shell kpsexpand '$$TEXMFHOME')


###########
# Archive #
###########

ARCHIVE_ROOT = $(FONT_NAME)
ARCHIVE = $(FONT_NAME).zip


###########
# Sources #
###########

TRUETYPE_FILES = $(wildcard *.ttf)

# Fontinst files
FONTINST_FILE = $(FONT_NAME)-drv.tex
FONTINST_MAP_FILE = $(FONT_NAME)-map.tex

# Custom Fontinst encoding files
INPUT_ETX_FILES = $(FONT_NAME)-01.etx $(FONT_NAME)-02.etx $(FONT_NAME)-dotlessj.etx
MTX_FILES = $(FONT_NAME)-fixlatin.mtx $(FONT_NAME)-fixtextcomp.mtx

STYLE_FILES = $(wildcard *.sty)

DOCUMENTATION = $(FONT_NAME).tex $(FONT_NAME).pdf $(FONT_NAME)-samples.tex $(FONT_NAME)-samples.pdf README CHANGES

# Files to be installed in texmf/source
SOURCE_FILES = $(FONTINST_FILE) $(FONTINST_MAP_FILE) $(INPUT_ETX_FILES) $(MTX_FILES) Makefile ttf2type1.pe


###################
# Generated files #
###################

TYPE1_FILES = $(TRUETYPE_FILES:.ttf=.pfb) $(TRUETYPE_FILES:.ttf=-LCDFJ.pfb)
AFM_FILES = $(TYPE1_FILES:.pfb=.afm)

# Fontinst log file
FONTINST_REC_FILE = $(FONT_NAME)-rec.tex

# Metrics files
PL_FILES = $(foreach e,$(INPUT_ENCODINGS),   \
             $(TRUETYPE_FILES:.ttf=-$(e).pl) \
           )
OUTPUT_MTX_FILES = $(PL_FILES:.pl=.mtx)
VPL_FILES = $(foreach e,$(SUPPORTED_ENCODINGS),          \
              $(TRUETYPE_FILES:.ttf=-$(e).vpl)           \
            )                                            \
            $(foreach e,$(SUPPORTED_SC_ENCODINGS),       \
              $(TRUETYPE_FILES:.ttf=-SmallCaps-$(e).vpl) \
            )
TFM_FILES = $(PL_FILES:.pl=.tfm) $(VPL_FILES:.vpl=.tfm)
VF_FILES = $(VPL_FILES:.vpl=.vf)

MAP = $(FONT_NAME).map

# Font definition files
FD_FILES = $(foreach e,$(SUPPORTED_ENCODINGS), \
             $(foreach f,$(FONT_CODES),        \
               $(e)$(f).fd                     \
             )                                 \
           )

# Generated encoding files
ENC_FILES = $(INPUT_ETX_FILES:.etx=.enc)

# Generated files to be installed
GENERATED_FILES = $(TYPE1_FILES) $(AFM_FILES) $(TFM_FILES) $(VF_FILES) $(MAP) $(FD_FILES) $(ENC_FILES)


default: all


all: dist


dist: $(ARCHIVE)


%.pfb %.afm: %.ttf
	fontforge ttf2type1.pe $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%-LCDFJ.pfb: %.pfb
	t1dotlessj $< $@


%-LCDFJ.afm: %-LCDFJ.pfb
	pf2afm $<
	# BUGFIX: fix FontName to the name of the file
	sed -i "s/^FontName .*/FontName $*/" $*.afm


%.tfm: %.pl
	pltotf $< $@


%.tfm: %.vpl
	vptovf $^ $


%.vf: %.vpl
	vptovf $^ $@


$(FONTINST_REC_FILE): $(AFM_FILES) $(MTX_FILES) $(FONTINST_FILE)
	latex $(FONTINST_FILE)


$(PL_FILES) $(VPL_FILES): $(FONTINST_REC_FILE)


$(MAP): $(FONTINST_REC_FILE) $(FONTINST_MAP_FILE)
	latex $(FONTINST_MAP_FILE)


$(FD_FILES) $(ENC_FILES): $(MAP)


texmf-tree: clean-texmf-tree $(GENERATED_FILES) $(SOURCES_FILES)
	mkdir -p $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/fonts/{afm,tfm,truetype,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	mkdir -p $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p $(DOCUMENTATION) $(ARCHIVE_ROOT)/doc/fonts/$(FONT_NAME)/
	cp -p $(FD_FILES) $(STYLE_FILES) $(ARCHIVE_ROOT)/tex/latex/$(FONT_NAME)/
	cp -p $(ENC_FILES) $(ARCHIVE_ROOT)/fonts/enc/dvips/$(FONT_NAME)/
	cp -p $(MAP) $(ARCHIVE_ROOT)/fonts/map/dvips/$(FONT_NAME)/
	cp -p $(AFM_FILES) $(ARCHIVE_ROOT)/fonts/afm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TFM_FILES) $(ARCHIVE_ROOT)/fonts/tfm/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TRUETYPE_FILES) $(ARCHIVE_ROOT)/fonts/truetype/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(TYPE1_FILES) $(ARCHIVE_ROOT)/fonts/type1/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(VF_FILES) $(ARCHIVE_ROOT)/fonts/vf/$(FOUNDRY)/$(FONT_NAME)/
	cp -p $(SOURCE_FILES) $(ARCHIVE_ROOT)/source/fonts/$(FONT_NAME)/
	cp -p README $(ARCHIVE_ROOT)
	cd $(ARCHIVE_ROOT) && find . -type f > manifest.txt


$(ARCHIVE): clean-texmf-tree texmf-tree
	zip -r $@ $(ARCHIVE_ROOT)


install: texmf-tree
	mkdir -p $(TEXMFHOME)
	cp -a $(ARCHIVE_ROOT)/* $(TEXMFHOME)
	texhash
	updmap --enable Map=$(MAP)


uninstall:
	$(RM) -r $(TEXMFHOME)/doc/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/tex/latex/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{enc,map}/dvips/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/fonts/{afm,tfm,type1,vf}/$(FOUNDRY)/$(FONT_NAME)/
	$(RM) -r $(TEXMFHOME)/source/$(FONT_NAME)/
	updmap --disable $(MAP)
	texhash


clean: clean-texmf-tree
	$(RM) $(TYPE1_FILES) $(AFM_FILES)
	$(RM) $(FONTINST_REC_FILE)
	$(RM) $(PL_FILES) $(TYPE1_FILES:.pfb=.pl)
	$(RM) $(OUTPUT_MTX_FILES) $(TYPE1_FILES:.pfb=.mtx)
	$(RM) $(VPL_FILES)
	$(RM) $(TFM_FILES)
	$(RM) $(VF_FILES)
	$(RM) $(MAP)
	$(RM) $(FD_FILES)
	$(RM) $(ENC_FILES)
	$(RM) $(ARCHIVE)
	$(RM) *~ *.log


clean-texmf-tree:
	$(RM) -r $(ARCHIVE_ROOT)


.PHONY: clean clean-texmf-tree texmf-tree

